FlintKV: A Fast Durable Storage Engine for Modern Databases

Byte-addressable non-volatile memory (NVM) offers an opportunity to rethink storage engine architectures. While recent NVM key-value stores achieve high throughput for ingestion and point lookups, they omit or under-specify the support for the richer interface guarantees required by modern databases. Production key-value engines (e.g., RocksDB) provide point-in-time snapshots, consistent iterators, and atomic batches-features essential for implementing transactions and concurrency control. We present FlintKV, an NVM-optimized skiplist-based storage engine that natively supports the full API of production key-value stores. FlintKV supports both atomic batch writes and snapshot-consistent iteration efficiently while guaranteeing durable linearizability. FlintKV can be deployed standalone or its durable skiplist can be integrated into existing NVM stores to enhance their capabilities. Central to FlintKV is a novel flat-combining based concurrency control algorithm that leverages multi-versioning and carefully co-designed persistence mechanisms to ensure high performance and scalability. Our empirical evaluation shows that FlintKV can achieve up to a 75% improvement in end-to-end throughput over prior work.

==> locals-style.tex <==
% Local style overrides and helper macros
% ParticipantArgs field macros: use these to keep field names/types consistent
% Usage examples:
%   \PAstate -> expands to the state field
%   \PAinode -> expands to the i_node field
%   \ParticipantArgsFields -> expands to a short description of all fields
\newcommand{\PAstate}{state}
\newcommand{\PAinode}{i\_node}
\newcommand{\PApreds}{preds}
\newcommand{\PAsuccs}{succs}
\newcommand{\PAcallback}{callback}
\newcommand{\PAresult}{result}
\newcommand{\ParticipantArgsFields}{\PAstate, \PAinode, \PApreds, \PAsuccs, \PAcallback, \PAresult}

\newcommand{\ParticipantArgs}{ParticipantArgs\xspace}
\newcommand{\ParticipantArgst}{\texttt{ParticipantArgs}\xspace}
\newcommand{\LocalThreadId}{tid}
\newcommand{\LocalThreadIdt}{\texttt{tid}}
\newcommand{\LocalThreadIdX}{tid\xspace}
\newcommand{\LocalThreadIdXt}{\texttt{tid}\xspace}

% PMEM-resident global variables

\newcommand{\useCommitEntry}{batch\_mode\xspace}
\newcommand{\useCommitEntryt}{\texttt{batch\_mode}\xspace}
\newcommand{\commitSeqId}{commit\_version\xspace}
\newcommand{\commitSeqIdt}{\texttt{commit\_version}\xspace}

% PMEMNode fields
\newcommand{\PMnext}{next\xspace}
\newcommand{\PMseqId}{seq\_id\xspace}
\newcommand{\PMkeyData}{key}
\newcommand{\PMValue}{value}

% IndexNode fields
\newcommand{\INnextPtrs}{next\_ptrs\xspace}
\newcommand{\INseqId}{seq\_id\xspace}
\newcommand{\INbaseNode}{p\_node}
\newcommand{\INheight}{height\xspace}
\newcommand{\INkeyHandle}{key}


% DRAM-resident global variables
\newcommand{\visibleSeq}{visible\_version\xspace}
\newcommand{\visibleSeqt}{\texttt{visible\allowbreak\_version}\xspace}
\newcommand{\gParticipants}{participants\xspace}
\newcommand{\gAdvertisements}{advertisements}
\newcommand{\gAdvertisementsX}{advertisements\xspace}
\newcommand{\gParticipantst}{\texttt{participants}\xspace}
\newcommand{\gParticipantsVar}{participants\xspace} % bare name for use in expressions/loops

\newcommand{\PUT}{PUT\xspace}
\newcommand{\GET}{GET\xspace}
\newcommand{\WriteBatch}{WriteBatch\xspace}
\newcommand{\InsertCallback}{\Op{insert}\xspace}
\newcommand{\ProcessPut}{\Op{Process\_Put}}
\newcommand{\ProcessPutX}{\Op{Process\_Put}\xspace}
\newcommand{\MultiKeyInsertCallback}{\Op{multikey\_insert}\xspace}
\newcommand{\callback}{callback\xspace}
\newcommand{\SnapshotIterator}{Snapshot Iterator\xspace}

\newcommand{\entriesLength}{entriesLength\xspace}
\newcommand{\batchEntries}{batchEntries\xspace}
\newcommand{\BatchEntries}{BatchEntries\xspace}
\newcommand{\pargs}{pargs\xspace}
\newcommand{\NVMM}{NVM\xspace}
\newcommand{\durableStagingTier}{durable staging tier\xspace}
\newcommand{\stagingTier}{staging tier\xspace}
\newcommand{\capacityTier}{capacity tier\xspace}
\newcommand{\str}{string\xspace}
\newcommand{\IndexNode}{IndexNode\xspace}
\newcommand{\batchModeX}{batch\_mode \xspace}
\newcommand{\batchMode}{batch\_mode}

\newcommand{\Op}[1]{{\sc \capitalisewords{\lowercase{#1}}}}
\newcommand{\Optt}[1]{\Op{#1}}%{\tt \lowercase{#1}}}

\newcommand{\througputFirstSet}{300K\xspace}
\newcommand{\througputSecondSet}{1M\xspace}
\newcommand{\througputThirdSet}{2M\xspace}
\newcommand{\fixedPayloadSizeForTheFirstBenchSet}{64B\xspace}
\newcommand{\fixedNumOpsForTheThirdBenchSet}{250K\xspace}
\newcommand{\pmemRocksDB}{PmemRocksDB\xspace}
\newcommand{\prdbX}{PMemRocksDB\xspace}
\newcommand{\prdb}{PMemRocksDB\xspace}
\newcommand{\kv}{KV}
\newcommand{\kvx}{KV\space}

\newcommand{\lookupKey}{key\xspace}

\newcommand{\MAXUINT}{{\tt MAX\_UINT}\xspace}
\newcommand{\fast}{$\mathbin{\color{dgreen}\bullet}$}  % green dot
\newcommand{\slow}{$\mathbin{\color{red}\bullet}$}    % red do

\newcommand{\persistr}{{\tt persist\_range}\xspace}
%\newcommand{\persist2}[2]{{\tt persist\_range(}#1, #2{\tt )}\xspace}
\newcommand{\flushr}{{\tt flush\_range}\xspace}
%\newcommand{\flushp}[2]{\texttt{flush\_range(}#1,#2{\tt )}}



